Adaptive Community Search in Dynamic Networks

Community search is a well-studied problem which, given a static graph and a query set of vertices, requires to find a cohesive (or dense) subgraph containing the query vertices. In this paper we study the problem of community search in temporal dynamic networks. We adapt to the temporal setting the notion of \emph{network inefficiency} which is based on the pairwise shortest-path distance among all the vertices in a solution. For this purpose we define the notion of \emph{shortest-fastest-path distance}: a linear combination of the temporal and spatial dimensions governed by a user-defined parameter. We thus define the \textsc{Minimum Temporal-Inefficiency Subgraph} problem and show that it is \NPhard. We develop an algorithm which exploits a careful transformation of the temporal network to a static directed and weighted graph, and some recent approximation algorithm for finding the minimum Directed Steiner Tree. We finally generalize our framework to the streaming setting in which new snapshots of the temporal graph keep arriving continuously and our goal is to produce a community search solution for the temporal graph corresponding to a sliding time window.

==> algorithms.tex <==
\begin{figure*}[t!]
	\centering
	%\includegraphics[width =0.8\textwidth ]{figures/process.pdf}
	\includegraphics[width =\textwidth ]{figures/phase1_four_graphs.pdf}
	%\includegraphics[width =0.8\textwidth ]{figures/phase1.pdf}
	\caption{Example of window graph $\textbf{G}_W$ with $|W|=2$ (left), its corresponding transformed graph $G'$ and the transitive closure computation process (right).}\label{fig:transformation}
\end{figure*}
In this section we introduce our method for computing the \emph{minimum inefficiency dynamic subgraph}, given as input a window graph $\textbf{G}_W$, a set of query vertices $Q$, and a user-defined parameter $\alpha \in [0,1]$. To this end, we need to compute a dynamic connector $\mathcal{H}_W$ that connects all of $Q$ in the window $W$ and then iteratively remove non-query vertices, as long as, by removing them, the inefficiency is reduced.

Our approach consists of three phases. In the first phase we initially transform the dynamic graph (inspired by~\cite{HuangFL15}), defined by the graph window, to a static graph by linking the various replicas of the same vertex in different timestamps and appropriately weighting these edges and the original edges. Afterwards, we compute the transitive closure of the transformed graph which will be used in the next phase. In the second phase, we compute the dynamic Steiner tree with the minimum cost that connects all query vertices of $Q$ in the window $W$. For this we use the notion of shortest-fastest paths and we employ the graph transformation to efficiently compute the minimum Steiner tree. Following, we extract the dynamic connector $\mathcal{H}_W$, that is induced by the minimum Steiner tree. In the final phase, starting from the subgraph computed in phase two, we find the \emph{minimum inefficiency dynamic subgraph} by applying a greedy relaxing algorithm. Next, we describe formally and in detail the three phases of our approach.

\spara{Phase 1: Graph Transformation.}
\begin{algorithm}[t!]
	\caption{GraphTransformation}\label{algo:Graph_transformation}
	\Input {$\textbf{V}_W = \bigcup_{i \in W} V_i$, $\textbf{E}_W =  \bigcup_{i \in W} E_i$, $\alpha$, $Q$, $Q'$, $W$}
	\Output {Transformed graph $G'$}	
	$V'$ \define $\bigcup\{(v,t): v \in V_t, t \in W\}$\label{line:start_transformation} \Comment{vertex renaming}
	$E'$ \define $\bigcup\{((v,t), (u,t), \alpha): v,u \in V_t, t \in W\}$ \Comment{static edges}
	$E'$ \define $E' \cup \{((v,t), (u,t'), (t'-t)(1-\alpha)): (v,t), (v,t') \in V', t'= \min\{t_i:(v,t_i)\in V', t_i>t\}\}$\label{line:finish_transformation} \Comment{temporal edges}	
	%$V'$ \define $V' \cup \{(u,-1): u \in Q\}$\;
	$V'$ \define $V' \cup Q' \cup Q$\label{line:start_augmented}\Comment{adds dummy source and destination vertices}
	$E'$ \define $E' \cup \{(u,(u,t),0): (u,t) \in V', u\in Q\}$ \Comment{connect dummy source vertices}
	$E'$ \define $E' \cup \{((u,t),(u,-1),0): (u,t) \in V', (u,-1) \in Q'\}$\label{line:finish_augmented} \Comment{connect dummy destination vertices}
	
	%$G' = (V',E')$\;	
	\Return {$G'= (V',E')$}
\end{algorithm}

Given a window graph $\textbf{G}_W = (\textbf{V}_W,\textbf{E}_W)$, we transform it to a static, directed and weighted graph  $G'(V',E',r)$, where $r$ is the weighting function, as follows:
%and a dynamic unweighted graph within this window $\textbf{G}(\textbf{V},\textbf{E})=\ <G_{t_0},...,G_{t_{W-1}}>$ we convert it to a new graph $\textbf{G}'(\textbf{V}', \textbf{E}', r)$ where $r: E' \rightarrow \{\alpha, 1-\alpha\}$ is the weight function, by following the next steps:
\squishenum
\item \textbf{Vertices:} for each $t \in W$, $v \in V_t$ we create a vertex id as a pair vertex-timestamp $(v,t)$, i.e., $V' = \{(v,t): t \in W, v \in V_{t}\}$.
%\item Vertex creation: for each snapshot $t$ of the graph that expands within the graph window and for each vertex $v$ of the snapshot $t$ we create a new vertex identified by the tuple of the id of the vertex and the timestamp that it appeared i.e. $(v,t)$. More formally we have that $\textbf{V}' = \{(v,t_i): v \in V_{t_i}, 0 \leq i \leq W-1 \}$ where $V_{t_i}$ is the set of vertexs of $G_{t_i}$ and $G_{t_i} \in \textbf{G}$.
\item \textbf{Edges:} for each $v \in V$  and each pair of timespans $t_i, t_j \in W$ with $t_j = min\{t: (v,t) \in V', t > t_i\}$, we create a directed edge $((v,t_i),(v,t_j))$ with weight $(t_j - t_i) (1 - \alpha)$. The edges in $\textbf{E}_W$, are instead assigned a weight of $\alpha$.
\squishend
Algorithm~\ref{algo:Graph_transformation} (lines~\ref{line:start_transformation}-~\ref{line:finish_transformation}) describes the graph transformation process. In Figure~\ref{fig:transformation} (left-middle) we see a window graph and its corresponding transformed graph.

Let us consider now a pair of vertices $(u,v) \in V \times V$, and let us define $P(u,v) = \{p((u,t_i),(v,t_j)) | t_i, t_j \in W \}$ the set of all paths from any replica of $u$ to any replica of $v$ in the transformed graph $G'$. Let us also denote $\ell(p)$ the length of one such path $p$, i.e., the sum of the weights of the edges in the path. Thanks to the edge labeling in $G'$, the following (straightforward) lemma holds.
\begin{lemma}
	A path $p$ on the transformed graph $G'$  from a replica of $u$ to a replica of $v$, corresponds to a valid temporal path $p'$ from $u$ to $v$ in the window graph $\textbf{G}_W$, and the length of $p$ in $G'$ corresponds to the cost of $p'$ in  $\textbf{G}_W$, i.e.,  $$\ell(p) = \mathcal{L}(p').$$
\end{lemma}
Following this observation, our method aims at computing the transitive closure of the window graph  $\textbf{G}_W$ which corresponds to the transitive closure of the transformed graph $G'$. For this, we compute for each pair of vertices $(u,v) \in V \times V$, the length of the shortest path from any replica of $u$ to any replica of $v$ (and viceversa), on the transformed graph $G'$.




Let $\ell^*(u,v) = \argmin_{p \in P(u,v)} \ell(p)$. We want to compute the length of the path $|SP(u,v)|$, where $SP(u,v)  = \{p \in P(u,v) | \ell(p) =  \ell^*(u,v)\}, \forall (u,v) \in V \times V$.
In order to compute the length of the shortest path from any replica of $u$ to any other vertex in $G'$, we create a dummy source vertex $u$ and connect it to all the replicas of $u$ in $G'$ by means of directed arcs with weight of 0. An example of computation of the shortest path that starts from the vertex with id $0$ is shown in Figure~\ref{fig:transformation} (right). In this case we need to concurrently calculate all shortest path from the vertices $(0,0)$ and $(0,1)$. Therefore, we run Dijkstra's algorithm starting from the dummy source vertex $0$ as source, returning only the length of the shortest paths to the rest of the vertices of $G'$.

\begin{figure*}[t!]
	\centering
	\includegraphics[width =\textwidth ]{figures/steiner_trees_four_graphs.pdf}
	%\includegraphics[width =\textwidth ]{figures/steiner_trees.pdf}
	\caption{Possible dynamic Steiner trees of a window graph with terminal vertices $[(0,-1),(4,-1),(1,-1)]$, depending on $\alpha$. On the left and middle part of the figure we see the possible dynamic Steiner trees rooted at $0$ when $\alpha<0.5$. On the right part of the figure we se the dynamic Steiner tree when $\alpha >0.5$. Finally, when $\alpha=0$ all three trees are dynamic Steiner trees of the graph.}\label{fig:steiner_trees}
\end{figure*}

\begin{mytheorem}\label{theorem:phantom}
	Running Dijkstra's algorithm from dummy source vertex $u$ correctly finds the set of all the shortest paths from any replica of $u$ to a vertex $(v,t) \in V'$ .
\end{mytheorem}

\begin{proof}
	First we observe that in a shortest path $p(u,(v,t))$ there is at most one intermediate vertex from the set $\{(u,t'): t' \in W\}$, that can by proved by absurd. Therefore, a shortest path from a dummy source vertex $u$ to a vertex $(v,t) \in V'$ will be $p(u,(v,t)) = \langle u,(u,t_i), x_i..., (v,t)\rangle$ where $x_i \neq (u,t_j)$ for any $t_j \in W$. Using Bellman Criterion on shortest paths of static graphs~\cite{Brandes01afaster}, we have that the shortest path from $(u,t_i)$ to $(v,t)$ can be obtained by removing $u$ from the path $p(u,(v,t))$.
\end{proof}

Let us go back to the example of Figure~\ref{fig:transformation}. In our attempt to calculate the SFP from vertex with id $0$ to the vertex with id $5$ we can run some shortest path algorithm starting from the dummy source vertex $0$ of the transformed graph.
%Figure~\ref{fig:transformation} (third graph) shows the computation of the SFPs from the vertex with id $0$. Let us consider the case of the SFP from vertex with id $0$ to the vertex with id $5$.
The algorithm detects a shortest path in timestamp zero and in timestamp one, with length $3\alpha$ and $\alpha$, respectively (marked in red). Up to this point, vertex $(5,0)$ and $(5,1)$ are treated as different vertices. However, these are the two versions of the vertex with id $5$ and therefore, the algorithm should choose the shortest path among them which corresponds to the SFP. For this, we augment the transformed graph with a dummy destination vertex $(5,-1)$ and we connect all the versions of the vertex with id $5$ with directed arcs with zero weight, as shown in Figure~\ref{fig:transformation} (fourth graph). The shortest path from dummy source vertex $u \in V'$ to the dummy destination vertex $(v,-1) \in V'$ corresponds to the SFP between vertices $u \in \textbf{V}_W$ and $v \in \textbf{V}_W$.


\begin{mytheorem}\label{theorem:source_destination_dummy}
	The shortest path from a dummy source vertex $u$ to a dummy destination vertex $(v,-1)$ on the augmented transformed graph $G'$ corresponds to the SFP from the vertex $u \in \textbf{V}_W$ to the vertex $v \in \textbf{V}_W$.
\end{mytheorem}

In the last part of phase 1 we augment the transformed graph $G'$ with a dummy source vertex and a dummy destination vertex for each one of the query vertices $Q$. Let us call $Q'$ the set of the dummy destination vertices. Algorithm~\ref{algo:Graph_transformation} (lines~\ref{line:start_augmented}-~\ref{line:finish_augmented}) describes the above process. The importance of the dummy source and destination vertices will result useful for the next phases of the process.

Depending on the value of the parameter $\alpha$ the SFPs between two vertices can vary significantly. Consider the example of Figure~\ref{fig:transformation} (third graph) and the pair of vertices with id (in the original graph) $0$ and $4$. The SFP from vertex with id $0$ to vertex with id $4$ can come from both timestamp zero and one, when $\alpha <0.5$ (paths highlighted with blue color). In this case, there are four SFPs from vertex $0$ to vertex $4$ all of which have length $3\alpha$. However, if $\alpha >0.5$ the SFP will expand to both timestamps zero and one (path highlighted with green color) with length $1+\alpha$. Finally, when $\alpha=0.5$ all the previous paths (blue and green paths) are SFPs.




\spara{Phase 2: Dynamic Steiner Tree.} Our next objective is to find a connector $\mathcal{H}_W$ that connects all vertices of $Q$. To this end, we compute the \emph{minimum dynamic Steiner tree}, from which we induce the dynamic connector $\mathcal{H}_W$. But first let us recall the definition of the \emph{minimum Steiner tree} in static graphs:


\begin{definition}[Minimum Steiner Tree in Static Graphs]
	Let $G=(V,E,w)$ be a static weighted graph, where $V$ is the set of vertices, $E =\{(u,v): u,v \in V\}$ is the set of edges and $w: V\times V \rightarrow [0,1]$ is the weighting function of the edges. Given a set of terminal vertices $Q\subset V$ and a root vertex $r$, we call Steiner Tree $T$ the tree rooted at vertex $r$ and contains a path from $r$ to every $q \in Q$. We call \emph{minimum Steiner Tree} $T^* = (V_T,E_T)$ the Steiner Tree that minimizes the cost $C_T =  \sum_{(u,v) \in E_T}w(u,v)$.

\end{definition}

Following, we extend the definition of the minimum Steiner tree to the case of dynamic graphs:
\begin{definition}[Minimum Dynamic Steiner Tree]
	Let us now consider a window graph $\textbf{G}_W = (\textbf{V}_W,\textbf{E}_W)$. Given a set of terminal vertices $Q \subset V_W$ and a root vertex $r \in V_W$, we call dynamic Steiner tree $\textbf{T}_W$, the tree rooted at $r$ which contains valid temporal paths from $r$ to every $q \in Q$. We call \emph{minimum dynamic Steiner Tree} the tree $\textbf{T}^*_W = (V_{\textbf{T}_W},E_{\textbf{T}_W})$ that minimizes the cost $C_{\textbf{T}_W} = | E_{\textbf{T}_W}|$.% \sum_{(u,v) \in E_{\textbf{T}_W}}w(u,v)$
	
\end{definition}

According to Lemma~\ref{lemma1} a dynamic Steiner tree on a window graph  $\textbf{G}_W$ corresponds to a static Steiner tree on the transformed graph $G'$. Therefore, our objective is to calculate the minimum Steiner tree on the transformed graph, that connects every $q \in Q$. To this end, we select a vertex $q_i \in Q$ as root vertex and as terminals the vertices in $Q'$ and we employ a modification of the approximation algorithm described by~\cite{HuangFL15}.
%The process starts by creating a dummy source vertex for the root vertex $r$ and connect it with directed edges with weight $0$ to all versions of the $r$ in $G'$. Next, for each vertex $q \in Q$ we create a phantom vertex $(q,-1)$ and we connect each version of $q$ in $G'$ in terms of directed edges with weight $0$.
%Finally, we calculate the minimum Steiner tree with root the dummy source vertex $r$ and terminal vertices the set $Q'=\{(q,-1): q \in Q\}$.

Figure~\ref{fig:steiner_trees} shows the process described above in order to compute the minimum Steiner tree with root vertex $0$ and terminal vertices $Q'=[(0,-1),(1,-1),(4,-1)]$. We repeat the process, choosing each time a different root vertex $r \in Q$. Finally, we choose as minimum Steiner tree $T$ the tree that has the minimum cost among the resulting Steiner trees $T_r$ with $r\in Q$.
\todo{include case disconnected dataset}

Similarly to the case of SFPs, minimum Steiner trees can vary depending on the value of the parameter $\alpha$. Figure~\ref{fig:steiner_trees} (second to last graph), shows the resulting Steiner trees, with root vertex $0$ and terminal vertices $Q'=[(0,-1),(1,-1),(4,-1)]$, when varying the value of the parameter $\alpha$. The second and the third graph of Figure~\ref{fig:steiner_trees} shows the two minimum Steiner trees when $\alpha<0.5$. When $\alpha>0.5$, the fourth graph is the only minimum Steiner tree. Finally, when $\alpha=0.5$, all three Steiner trees are minimum Steiner trees.

The last step of phase 2 is the computation of the steiner connector which is induced by the minimum Steiner tree $T$.
We have that $H=(V_{H},E_{H})$ where $V_{H}=\{(v,t)| (v,t)\in V', \exists t_i in W: (v,t_i) \in T\}$ and $E_{H}=\{(v,u) \in E' | v\in V_{H}, u\in V_{H}\}$. Finally, the dynamic connector $\mathcal{H} = (V_\mathcal{H},E_\mathcal{H})$  where $V_\mathcal{H} = \{v \in \textbf{V}_W| \exists t \in W: (v,t) \in V_{H}\}$ and $E_\mathcal{H}=\{(u,v) \in \textbf{E}_W| \exists t_i,t_j \in W: ((u,t_i),(v,t_j)) \in E_{H}\}$.

\spara{Phase 3: Minimum Inefficiency Dynamic Subgraph.}
%\begin{figure*}[ht!]
%	\centering
%	\includegraphics[width =\textwidth ]{figures/Moving_window_update.pdf}
%	\caption{Transformed graph for 3 consecutive timestamps for $|W| = 3$. The  figure shows the second timestamp (Timestamp 1) where $W$ contains two snapshots of $\textbf{G}_W$. In the last instance of the figure we the most obsolete snapshot is removed from W for the newest one to enter}\label{fig:update_window}
%\end{figure*}

\begin{algorithm}[t!]
	\caption{Minimum Inefficiency Dynamic Subgraph}\label{algorithm:MIS}
	\Input{$W$, Window Graph $\textbf{G}_W = (\textbf{V}_W,\textbf{E}_W)$, $\alpha$, query vertices $Q\subseteq \textbf{V}_W$}
	%\Output{Selective connector $\textbf{G}_W[\textbf{S}_W]$ s.t. $Q\subseteq \textbf{S}_W \subseteq \textbf{V}_W$}
	\Output{Selective connector $\mathcal{H}_W$ s.t. $Q\subseteq V_\textbf{H}\subseteq \textbf{V}_W$}
		
	$Q'$ \define $\{(u,-1): u \in Q\}$\label{line:Q'}\Comment{dummy destination vertices}
	$G'$ \define GraphTransformation($\textbf{V}_W,\textbf{E}_W,\alpha,Q, Q', W$)\label{line:transformation} \Comment{Algorithm~\ref{algo:Graph_transformation}}
	$\mathbb{G}'$ \define Transitive closure of $G'$\label{line:transitive_closure}
	
	\For{$r \in Q$\label{line:start_stTree}}
	{
		$T_r$ \define MinimumSteinerTree($\mathbb{G}'$, $r$, $Q'$)

	}
	$T$ \define $\argmin_{r \in Q}$ cost$(T_r)$\label{line:minsteinerTree}
	\Comment{minimun Steiner tree $T=(V_T,E_T)$}
	%$\argmin_{r \in Q} MinimumSteinerTree($G'$, $r$, $Q'$)$
	%$T$ \define MinimumSteinerTree($G'$, $Q'$)\label{line:steinerTree}\;
	 %$\mathcal{H}_W$ \define inducedSubgraph($\textbf{G}_W$,$T$)\label{line:inducedSubgraph}\;
	 %$H'$ \define inducedSubgraph$(G',\mathcal{H}_W)$\;
	 $H$ \define $G'[T]$\label{line:steiner_connector} \Comment{steiner connector $H = (V_{H},E_{H})$  }
	
	 %$V_{H} = \{(v,t): (v,t)\in V', \exists t_i in W: (v,t_i) \in T\}$\;
	 %$E_{H}=\{(v,u) \in E' | v\in V_{H}, u\in V_{H}\}$\;
	
	
	 %$S$ \define $V_{H}$  \;
	$i$ \define $0$\;\label{line:greedy_start}
	\While{ $V_{H} \setminus \{(u,t): u \in Q\}$\label{line:while_loop}}{
		
		$\mathcal{H}_i$ \define $\textbf{G}_W[V_H]$ \label{line:induced_dynamic}\Comment{dynamic connector $\mathcal{H}_i=(V_{\mathcal{H}_i},E_{\mathcal{H}_i})$}
		
		$i$ \define $i +1$\;
		\For{$u \in \{V_{\mathcal{H}_i}\}$\label{line:for_loop}}{
			$c_u$ \define $\mathcal{I}(G'[V_H\setminus\{(u,t)\in V_H\}])$\;
		}
		$v$ \define $\argmin_{u} c_u$\;
		$V_H$ \define $V_H \setminus \{(v,t)\in V_H\}$	
	}
	$\mathcal{H}_W$ \define $\argmin_{j \in [0,i]} \mathcal{I}(\mathcal{H}_j)$\label{line:minimum_dynamic_connector}\;
	\Return{$\mathcal{H}_W$}\label{line:greedy_end}
\end{algorithm}
In the last phase of the process, starting with the steiner connector $H$, we compute the minimum inefficiency dynamic subgraph $\mathcal{H}_W$.
The algorithm iteratively removes from the sub-graph $H$ all vertices that do not appear in the query set.
$\mathcal{H}_W$, we compute the minimum inefficiency dynamic subgraph.
The algorithm, iteratively removes from the induced sub-graph all vertices that do not appear in the query set in a greedy manner and computes their inefficiency. Finally, it returns the sub-graph that minimizes the inefficiency.


 Algorithm~\ref{algorithm:MIS} describes phases 1-3. Lines~\ref{line:Q'} and~\ref{line:transformation} describe the creation of the dummy destination nodes and the graph transformation of the window graph of phase 1. Phase 2 is described in lines~\ref{line:transitive_closure} to~\ref{line:steiner_connector}. In the for loop of line~\ref{line:start_stTree} we compute the Steiner tree starting from each dummy source node (query node) with terminal vertices the dummy destination nodes $Q'$. The tree $T_r$ that minimizes the cost function among all $T_r$ with $r \in Q$ is chosen as the minimum Steiner tree (line~\ref{line:minsteinerTree}) from which we induce the steiner connector in line~\ref{line:steiner_connector}. Finally, phase 3 is described in lines~\ref{line:greedy_start} to~\ref{line:greedy_end}. In the while loop of line~\ref{line:while_loop} we compute greedily the inefficiency of each steiner connector while we remove each vertex (all the versions of each vertex) that are not contained in the query set $Q$. In line~\ref{line:induced_dynamic} we compute the dynamic connector induced by the static connector $H$ as described in phase 2. In the for loop of line~\ref{line:for_loop} we choose the vertex that, by removing it, minimizes the inefficiency each time.
 At the end of the while loop~\ref{line:minimum_dynamic_connector} we choose the dynamic connector with the minimum inefficiency and we return it at line~\ref{line:greedy_end}.



\subsection*{Sliding window case}

Next we will discuss the problem of computing the minimum inefficiency dynamic subgraph in the sliding window case. In this setting, we consider an infinite stream of input graphs. At each timestamp the input graph is the latest snapshot of the dynamic graph, that updates the window $W$. The window $W$ slides one position in order to include the new input and leave outside the most obsolete snapshot.
The process for the computation of the minimum inefficiency dynamic subgraph continues as described in the static window case. However, after the computation of the dynamic subgraph $\mathcal{H}^t_W$, we update the query set for the next round. $Q_{t+1} = Q_0 \bigcup V^t_{\mathcal{H}}$. If the subgraph $\mathcal{H}^t_W$ is disconnected, the query set of the next round is considered the $Q_0$.


\begin{algorithm}[t!]
	\caption{MIDS: sliding window case}\label{algorithm:MIS2}
	\Input{$W$, %Window Graph $\textbf{G}_W = (\textbf{V}_W,\textbf{E}_W)$,
		$\alpha$, query vertices $Q_0\subseteq \textbf{V}_W$}

	\Output{Selective connector $\mathcal{H}_W$ s.t. $Q\subseteq V_\textbf{H}\subseteq \textbf{V}_W$, $Q_{t+1}$}
	
	$\textbf{G}_W$ \define $[]$, $V'$ \define $\emptyset$\label{line:start_transformation1}, $E'$ \define $\emptyset$, $t$\define$0$\\
	\While {$t< rounds$}{
		
		
		\Read $G_t(V_t,E_t)$\Comment{Read new timestamp}
		$V' \define V' \cup \{(v,t): v \in V_t \}$\label{line:updatestart} \Comment{Vertex renaming}\label{line:graph_transf_sliding_begin}
		$V'$ \define $V' \setminus \{(v,t_i): t_i = t-(|W|-2)\}$\Comment{Remove obsolete nodes}
		$E' \define E' \cup \{((v,t),(u,t), \alpha): (v,t)\in V', (u,t) \in V'$ and $(v,u) \in E_t \}$ \Comment{static edges}
		$E' \define E' \cup \{((v,t'),(v,t),(1-\alpha)(t-t'))\}$, where $t'= max\{t_i: (v,t_i) \in V', t_i < t\}$ \Comment{temporal edges}\label{line:graph_transf_sliding_end}
		$E' \define E' \setminus \{((v,t_i),(u,t_j)): t_i = t-(|W|-2)\}$\Comment{Remove obsolete edges}
		$V'$ \define $V' \cup Q'_t \cup Q_t$\label{line:start_augmented2}\Comment{adds dummy source and destination vertices}
		$E'$ \define $E' \cup \{(u,(u,t),0): (u,t) \in V', u\in Q_t\}$\Comment{connect dummy source vertices}
		$E'$ \define $E' \cup \{((u,t),(u,-1),0): (u,t) \in V', (u,-1) \in Q'_t\}$\label{line:finish_augmented2}\Comment{connect dummy destination vertices}
	$Q'_t$ \define $\{(u,-1): u \in Q_t\}$\label{line:Q'2}\Comment{dummy destination vertices}
	
	\textbf{Algorithm~\ref{algorithm:MIS} lines~\ref{line:transitive_closure}-~\ref{line:minimum_dynamic_connector}}\;
	\If {$E_{\mathcal{H}} \neq \emptyset$}{
	$Q_{t+1}$ \define $Q_0 \bigcup \{u\in V_{\mathcal{H}}: \exists v \in V_{\mathcal{H}}:  (u,v) \in E_{\mathcal{H}} \}$
	}
	\Else{ $Q_{t+1}$ \define $Q_0$}
	\Report{$\mathcal{H}_W$, $Q_{t+1}$}\label{line:greedy_end2}\;
	$t$ \define $t+1$
}
\end{algorithm}

%%TODO change this paragraph because it is copied from the previous paper.
%Figure~\ref{fig:update_window} shows the case of a sliding window of length 3 in three consecutive timestamps. Timestamp 0, which does not appear in the  figure, contains only the  first snapshot of the graph in the rightmost position of the window. Timestamp 1 (left side of Figure 3) shows the window after the appearance of the second snapshot of the graph. Therefore, the  first snapshot moves one position to the left of the window and gives its position to the new timestamp. Finally, we create the links between the vertices with same ids in the different timestamps. In the next timestamp, when a new snapshot arrives, occupies the rightmost position of the window, whereas, the older snapshots move one position to the left. If all the positions of the window are occupied, the oldest snapshot is removed from the window graph, as shown in the right part of Figure 3 marked with red color (Timestamp 3).

\subsection*{Distributed implementation}
For the computation of the Steiner tree as described in~\cite{HuangFL15} it is required some preprocessing in order to extract the transitive closure of the graph. For this, it is necessary to employ some computationally expensive algorithm like Floyd-Warshall, with computational complexity $\mathcal{O}(V^3)$. The complexity of the algorithm is high due to the computation of the transitive closure between all pairs of nodes. This adds to the streaming algorithms computational complexity which is prohibitive for large scale graph. In order to avoid this step, we exploit the properties of the algorithm and we calculate on the fly the transitive closure between two vertices in the graph, when this is required.
 To this end, instead of using Floyd-Warshall algorithm, we use Dijkstra's algorithm, and we calculate the shortest paths from a given source vertex to the rest of the vertices of the graph.

For the implementation of our algorithms we use the Apache Spark framework.
% \todo{Explain why not using Floyd-Warshall algorithm for the transitive closure calculation. Lazy evaluation for transitive closure. Distributed the computation of Steiner tree for each root vertex.}

